Modular Subgroups, Dessins d'Enfants and Elliptic K3 Surfaces

We consider the 33 conjugacy classes of genus zero, torsion-free modular subgroups, computing ramification data and Grothendieck's dessins d'enfants. In the particular case of the index 36 subgroups, the corresponding Calabi-Yau threefolds are identified, in analogy with the index 24 cases being associated with K3 surfaces. In a parallel vein, we study the 112 semi-stable elliptic fibrations over P^1 as extremal K3 surfaces with six singular fibres. In each case, a representative of the corresponding class of subgroups is identified by specifying a generating set for that representative.

==> PICT/111 <==
mv 10-10-1-1-1-1\ A.pdf 10-10-1-1-1-1_A.pdf;

mv 10-10-1-1-1-1\ B.pdf 10-10-1-1-1-1_B.pdf;

mv 10-10-1-1-1-1\ C.pdf 10-10-1-1-1-1_C.pdf;

mv 10-10-5-5-2-2-1-1.pdf 10-10-5-5-2-2-1-1.pdf;

mv 10-4-3-3-2-2.pdf 10-4-3-3-2-2.pdf;

mv 10-4-4-3-2-1.pdf 10-4-4-3-2-1.pdf;

mv 10-5-3-2-2-2.pdf 10-5-3-2-2-2.pdf;

mv 10-5-4-2-2-1\ A.pdf 10-5-4-2-2-1_A.pdf;

mv 10-5-4-2-2-1\ B.pdf 10-5-4-2-2-1_B.pdf;

mv 10-5-4-2-2-1\ C.pdf 10-5-4-2-2-1_C.pdf;

mv 10-5-5-2-1-1\ A.pdf 10-5-5-2-1-1_A.pdf;

mv 10-5-5-2-1-1\ B.pdf 10-5-5-2-1-1_B.pdf;

mv 10-6-3-2-2-1.pdf 10-6-3-2-2-1.pdf;

mv 10-6-4-2-1-1\ A.pdf 10-6-4-2-1-1_A.pdf;

mv 10-6-4-2-1-1\ B.pdf 10-6-4-2-1-1_B.pdf;

mv 10-6-5-1-1-1\ A.pdf 10-6-5-1-1-1_A.pdf;

mv 10-6-5-1-1-1\ B.pdf 10-6-5-1-1-1_B.pdf;

mv 10-6-5-1-1-1\ C.pdf 10-6-5-1-1-1_C.pdf;

mv 10-6-5-1-1-1\ D.pdf 10-6-5-1-1-1_D.pdf;

mv 10-7-2-2-2-1.pdf 10-7-2-2-2-1.pdf;

mv 10-7-3-2-1-1\ A.pdf 10-7-3-2-1-1_A.pdf;

mv 10-7-3-2-1-1\ B.pdf 10-7-3-2-1-1_B.pdf;

mv 10-7-4-1-1-1.pdf 10-7-4-1-1-1.pdf;

mv 10-8-3-1-1-1.pdf 10-8-3-1-1-1.pdf;

mv 10-9-2-1-1-1\ A.pdf 10-9-2-1-1-1_A.pdf;

mv 10-9-2-1-1-1\ B.pdf 10-9-2-1-1-1_B.pdf;

mv 11-4-3-3-2-1.pdf 11-4-3-3-2-1.pdf;

mv 11-4-4-3-1-1.pdf 11-4-4-3-1-1.pdf;

mv 11-5-3-2-2-1.pdf 11-5-3-2-2-1.pdf;

mv 11-5-3-3-1-1\ A.pdf 11-5-3-3-1-1_A.pdf;

mv 11-5-3-3-1-1\ B.pdf 11-5-3-3-1-1_B.pdf;

mv 11-5-4-2-1-1\ A.pdf 11-5-4-2-1-1_A.pdf;

mv 11-5-4-2-1-1\ B.pdf 11-5-4-2-1-1_B.pdf;

mv 11-5-4-2-1-1\ C.pdf 11-5-4-2-1-1_C.pdf;

mv 11-5-5-1-1-1.pdf 11-5-5-1-1-1.pdf;

mv 11-6-3-2-1-1\ A.pdf 11-6-3-2-1-1_A.pdf;

mv 11-6-3-2-1-1\ B.pdf 11-6-3-2-1-1_B.pdf;

mv 11-6-3-2-1-1\ C.pdf 11-6-3-2-1-1_C.pdf;

mv 11-6-4-1-1-1\ A.pdf 11-6-4-1-1-1_A.pdf;

mv 11-6-4-1-1-1\ B.pdf 11-6-4-1-1-1_B.pdf;

mv 11-7-2-2-1-1\ A.pdf 11-7-2-2-1-1_A.pdf;

mv 11-7-2-2-1-1\ B.pdf 11-7-2-2-1-1_B.pdf;

mv 11-7-3-1-1-1\ A.pdf 11-7-3-1-1-1_A.pdf;

mv 11-7-3-1-1-1\ B.pdf 11-7-3-1-1-1_B.pdf;

mv 11-7-3-1-1-1\ C.pdf 11-7-3-1-1-1_C.pdf;

mv 11-8-2-1-1-1\ A.pdf 11-8-2-1-1-1_A.pdf;

mv 11-8-2-1-1-1\ B.pdf 11-8-2-1-1-1_B.pdf;

mv 11-8-2-1-1-1\ C.pdf 11-8-2-1-1-1_C.pdf;

mv 11-9-1-1-1-1.pdf 11-9-1-1-1-1.pdf;

mv 12-12-6-4-4-3-3-2-1-1.pdf 12-12-6-4-4-3-3-2-1-1.pdf;

mv 12-3-3-2-2-2.pdf 12-3-3-2-2-2.pdf;

mv 12-3-3-3-2-1.pdf 12-3-3-3-2-1.pdf;

mv 12-4-3-2-2-1\ A.pdf 12-4-3-2-2-1_A.pdf;

mv 12-4-3-2-2-1\ B.pdf 12-4-3-2-2-1_B.pdf;

mv 12-4-3-2-2-1\ C.pdf 12-4-3-2-2-1_C.pdf;

mv 12-4-3-3-1-1\ A.pdf 12-4-3-3-1-1_A.pdf;

mv 12-4-3-3-1-1\ B.pdf 12-4-3-3-1-1_B.pdf;

mv 12-4-4-2-1-1.pdf 12-4-4-2-1-1.pdf;

mv 12-5-2-2-2-1.pdf 12-5-2-2-2-1.pdf;

mv 12-5-3-2-1-1\ A.pdf 12-5-3-2-1-1_A.pdf;

mv 12-5-3-2-1-1\ B.pdf 12-5-3-2-1-1_B.pdf;

mv 12-5-3-2-1-1\ C.pdf 12-5-3-2-1-1_C.pdf;

mv 12-5-3-2-1-1\ D.pdf 12-5-3-2-1-1_D.pdf;

mv 12-6-2-2-1-1\ A.pdf 12-6-2-2-1-1_A.pdf;

mv 12-6-2-2-1-1\ B.pdf 12-6-2-2-1-1_B.pdf;

mv 12-6-3-1-1-1.pdf 12-6-3-1-1-1.pdf;

mv 12-6-6-6-6-4-2-2-2-2.pdf 12-6-6-6-6-4-2-2-2-2.pdf;

mv 12-7-2-1-1-1\ A.pdf 12-7-2-1-1-1_A.pdf;

mv 12-7-2-1-1-1\ B.pdf 12-7-2-1-1-1_B.pdf;

mv 13-3-3-2-2-1.pdf 13-3-3-2-2-1.pdf;

mv 13-4-3-2-1-1.pdf 13-4-3-2-1-1.pdf;

mv 13-5-2-2-1-1\ A.pdf 13-5-2-2-1-1_A.pdf;

mv 13-5-2-2-1-1\ B.pdf 13-5-2-2-1-1_B.pdf;

mv 13-5-3-1-1-1.pdf 13-5-3-1-1-1.pdf;

mv 13-6-2-1-1-1\ A.pdf 13-6-2-1-1-1_A.pdf;

mv 13-6-2-1-1-1\ B.pdf 13-6-2-1-1-1_B.pdf;

mv 13-7-1-1-1-1.pdf 13-7-1-1-1-1.pdf;

mv 14-3-2-2-2-1.pdf 14-3-2-2-2-1.pdf;

mv 14-3-3-2-1-1\ A.pdf 14-3-3-2-1-1_A.pdf;

mv 14-3-3-2-1-1\ B.pdf 14-3-3-2-1-1_B.pdf;

mv 14-4-2-2-1-1\ A.pdf 14-4-2-2-1-1_A.pdf;

mv 14-4-2-2-1-1\ B.pdf 14-4-2-2-1-1_B.pdf;

mv 14-4-3-1-1-1.pdf 14-4-3-1-1-1.pdf;

mv 14-5-2-1-1-1\ A.pdf 14-5-2-1-1-1_A.pdf;

mv 14-5-2-1-1-1\ B.pdf 14-5-2-1-1-1_B.pdf;

mv 14-5-2-1-1-1\ C.pdf 14-5-2-1-1-1_C.pdf;

mv 14-5-2-1-1-1\ D.pdf 14-5-2-1-1-1_D.pdf;

mv 14-6-1-1-1-1\ A.pdf 14-6-1-1-1-1_A.pdf;

mv 14-6-1-1-1-1\ B.pdf 14-6-1-1-1-1_B.pdf;

mv 15-3-2-2-1-1\ A.pdf 15-3-2-2-1-1_A.pdf;

mv 15-3-2-2-1-1\ B.pdf 15-3-2-2-1-1_B.pdf;

mv 15-3-2-2-1-1\ C.pdf 15-3-2-2-1-1_C.pdf;

mv 15-3-2-2-1-1.pdf 15-3-2-2-1-1.pdf;

mv 15-3-3-1-1-1.pdf 15-3-3-1-1-1.pdf;

mv 15-4-2-1-1-1\ A.pdf 15-4-2-1-1-1_A.pdf;

mv 15-4-2-1-1-1\ B.pdf 15-4-2-1-1-1_B.pdf;

mv 15-5-1-1-1-1\ A.pdf 15-5-1-1-1-1_A.pdf;

mv 15-5-1-1-1-1\ B.pdf 15-5-1-1-1-1_B.pdf;

mv 16-16-2-2-2-2-2-2-2-2.pdf 16-16-2-2-2-2-2-2-2-2.pdf;

mv 16-16-4-4-2-2-1-1-1-1.pdf 16-16-4-4-2-2-1-1-1-1.pdf;

mv 16-2-2-2-1-1.pdf 16-2-2-2-1-1.pdf;

mv 16-3-2-1-1-1\ A.pdf 16-3-2-1-1-1_A.pdf;

mv 16-3-2-1-1-1\ B.pdf 16-3-2-1-1-1_B.pdf;

mv 16-3-2-1-1-1\ C.pdf 16-3-2-1-1-1_C.pdf;

mv 17-2-2-1-1-1\ A.pdf 17-2-2-1-1-1_A.pdf;

mv 17-2-2-1-1-1\ B.pdf 17-2-2-1-1-1_B.pdf;

mv 17-3-1-1-1-1.pdf 17-3-1-1-1-1.pdf;

mv 18-2-1-1-1-1\ A.pdf 18-2-1-1-1-1_A.pdf;

mv 18-2-1-1-1-1\ B.pdf 18-2-1-1-1-1_B.pdf;

mv 18-2-1-1-1-1\ C.pdf 18-2-1-1-1-1_C.pdf;

mv 2-2-2.pdf 2-2-2.pdf;

mv 25-25-1-1-1-1-1-1-1-1-1-1-1-1\ Attempt\ B.pdf 25-25-1-1-1-1-1-1-1-1-1-1-1-1_Attempt_B.pdf;

mv 25-25-1-1-1-1-1-1-1-1-1-1-1-1.pdf 25-25-1-1-1-1-1-1-1-1-1-1-1-1.pdf;

mv 32-8-1-1-1-1-1-1-1-1.pdf 32-8-1-1-1-1-1-1-1-1.pdf;

mv 4-1-1.pdf 4-1-1.pdf;

mv 4-4-2-2.pdf 4-4-2-2.pdf;

mv 4-4-4-4-4-4.pdf 4-4-4-4-4-4.pdf;

mv 5-5-1-1.pdf 5-5-1-1.pdf;

mv 5-5-4-4-3-3.pdf 5-5-4-4-3-3.pdf;

mv 5-5-5-5-2-2.pdf 5-5-5-5-2-2.pdf;

mv 5-5-5-5-5-5-5-5-5-5-5-5-5\ Attempt\ B.pdf 5-5-5-5-5-5-5-5-5-5-5-5-5_Attempt_B.pdf;

mv 5-5-5-5-5-5-5-5-5-5-5-5-5.pdf 5-5-5-5-5-5-5-5-5-5-5-5-5.pdf;

mv 6-3-2-1.pdf 6-3-2-1.pdf;

mv 6-5-4-4-3-2.pdf 6-5-4-4-3-2.pdf;

mv 6-6-3-3-3-3.pdf 6-6-3-3-3-3.pdf;

mv 6-6-4-3-3-2.pdf 6-6-4-3-3-2.pdf;

mv 6-6-4-4-2-2.pdf 6-6-4-4-2-2.pdf;

mv 6-6-5-3-3-1.pdf 6-6-5-3-3-1.pdf;

mv 6-6-5-4-2-1.pdf 6-6-5-4-2-1.pdf;

mv 6-6-5-5-1-1\ A.pdf 6-6-5-5-1-1_A.pdf;

mv 6-6-5-5-1-1\ B.pdf 6-6-5-5-1-1_B.pdf;

mv 6-6-6-2-2-2.pdf 6-6-6-2-2-2.pdf;

mv 6-6-6-4-1-1.pdf 6-6-6-4-1-1.pdf;

mv 7-5-4-3-3-2.pdf 7-5-4-3-3-2.pdf;

mv 7-5-4-4-3-1.pdf 7-5-4-4-3-1.pdf;

mv 7-5-5-3-2-2.pdf 7-5-5-3-2-2.pdf;

mv 7-5-5-4-2-1\ A.pdf 7-5-5-4-2-1_A.pdf;

mv 7-5-5-4-2-1\ B.pdf 7-5-5-4-2-1_B.pdf;

mv 7-6-4-4-2-1.pdf 7-6-4-4-2-1.pdf;

mv 7-6-5-3-2-1\ A.pdf 7-6-5-3-2-1_A.pdf;

mv 7-6-5-3-2-1\ B.pdf 7-6-5-3-2-1_B.pdf;

mv 7-6-5-3-2-1\ C.pdf 7-6-5-3-2-1_C.pdf;

mv 7-6-5-4-1-1.pdf 7-6-5-4-1-1.pdf;

mv 7-6-6-2-2-1.pdf 7-6-6-2-2-1.pdf;

mv 7-7-3-3-2-2\ A.pdf 7-7-3-3-2-2_A.pdf;

mv 7-7-3-3-2-2\ B.pdf 7-7-3-3-2-2_B.pdf;

mv 7-7-4-4-1-1\ B.pdf 7-7-4-4-1-1_B.pdf;

mv 7-7-4-4-1-1.pdf 7-7-4-4-1-1.pdf;

mv 7-7-5-3-1-1\ A.pdf 7-7-5-3-1-1_A.pdf;

mv 7-7-5-3-1-1\ B.pdf 7-7-5-3-1-1_B.pdf;

mv 7-7-7-1-1-1.pdf 7-7-7-1-1-1.pdf;

mv 8-2-1-1.pdf 8-2-1-1.pdf;

mv 8-4-4-4-2-2.pdf 8-4-4-4-2-2.pdf;

mv 8-4-4-4-3-1.pdf 8-4-4-4-3-1.pdf;

mv 8-5-4-3-2-2.pdf 8-5-4-3-2-2.pdf;

mv 8-5-4-3-3-1\ B.pdf 8-5-4-3-3-1_B.pdf;

mv 8-5-4-3-3-1.pdf 8-5-4-3-3-1.pdf;

mv 8-6-4-2-2-2.pdf 8-6-4-2-2-2.pdf;

mv 8-6-4-3-2-1\ A.pdf 8-6-4-3-2-1_A.pdf;

mv 8-6-4-3-2-1\ B.pdf 8-6-4-3-2-1_B.pdf;

mv 8-6-5-2-2-1.pdf 8-6-5-2-2-1.pdf;

mv 8-6-5-3-1-1\ A.pdf 8-6-5-3-1-1_A.pdf;

mv 8-6-5-3-1-1\ B.pdf 8-6-5-3-1-1_B.pdf;

mv 8-6-6-2-1-1\ A.pdf 8-6-6-2-1-1_A.pdf;

mv 8-6-6-2-1-1\ B.pdf 8-6-6-2-1-1_B.pdf;

mv 8-7-3-3-2-1.pdf 8-7-3-3-2-1.pdf;

mv 8-7-4-2-2-1\ A.pdf 8-7-4-2-2-1_A.pdf;

mv 8-7-4-2-2-1\ B.pdf 8-7-4-2-2-1_B.pdf;

mv 8-7-4-3-1-1\ A.pdf 8-7-4-3-1-1_A.pdf;

mv 8-7-4-3-1-1\ B.pdf 8-7-4-3-1-1_B.pdf;

mv 8-7-5-2-1-1\ A.pdf 8-7-5-2-1-1_A.pdf;

mv 8-7-5-2-1-1\ B.pdf 8-7-5-2-1-1_B.pdf;

mv 8-7-5-2-1-1\ C.pdf 8-7-5-2-1-1_C.pdf;

mv 8-7-6-1-1-1\ A.pdf 8-7-6-1-1-1_A.pdf;

mv 8-7-6-1-1-1\ B.pdf 8-7-6-1-1-1_B.pdf;

mv 8-8-2-2-2-2.pdf 8-8-2-2-2-2.pdf;

mv 8-8-3-3-1-1\ B.pdf 8-8-3-3-1-1_B.pdf;

mv 8-8-3-3-1-1\ C.pdf 8-8-3-3-1-1_C.pdf;

mv 8-8-3-3-1-1.pdf 8-8-3-3-1-1.pdf;

mv 8-8-4-2-1-1\ Attempt\ B.pdf 8-8-4-2-1-1_Attempt_B.pdf;

mv 8-8-4-2-1-1.pdf 8-8-4-2-1-1.pdf;

mv 8-8-4-4-4-4-4-4-4-4.pdf 8-8-4-4-4-4-4-4-4-4.pdf;

mv 8-8-8-8-4-4-2-2-2-2.pdf 8-8-8-8-4-4-2-2-2-2.pdf;

mv 9-4-3-3-3-2.pdf 9-4-3-3-3-2.pdf;

mv 9-5-3-3-3-1.pdf 9-5-3-3-3-1.pdf;

mv 9-5-4-3-2-1\ A.pdf 9-5-4-3-2-1_A.pdf;

mv 9-5-4-3-2-1\ B.pdf 9-5-4-3-2-1_B.pdf;

mv 9-5-4-3-2-1\ C.pdf 9-5-4-3-2-1_C.pdf;

mv 9-5-5-2-2-1.pdf 9-5-5-2-2-1.pdf;

mv 9-6-3-3-2-1\ A.pdf 9-6-3-3-2-1_A.pdf;

mv 9-6-3-3-2-1\ B.pdf 9-6-3-3-2-1_B.pdf;

mv 9-6-3-3-2-1\ C.pdf 9-6-3-3-2-1_C.pdf;

mv 9-6-4-3-1-1.pdf 9-6-4-3-1-1.pdf;

mv 9-6-5-2-1-1\ A.pdf 9-6-5-2-1-1_A.pdf;

mv 9-6-5-2-1-1\ B.pdf 9-6-5-2-1-1_B.pdf;

mv 9-6-5-2-1-1\ C.pdf 9-6-5-2-1-1_C.pdf;

mv 9-7-3-2-2-1\ A.pdf 9-7-3-2-2-1_A.pdf;

mv 9-7-3-2-2-1\ B.pdf 9-7-3-2-2-1_B.pdf;

mv 9-7-3-2-2-1\ C.pdf 9-7-3-2-2-1_C.pdf;

mv 9-7-4-2-1-1\ A.pdf 9-7-4-2-1-1_A.pdf;

mv 9-7-4-2-1-1\ B.pdf 9-7-4-2-1-1_B.pdf;

mv 9-7-5-1-1-1.pdf 9-7-5-1-1-1.pdf;

mv 9-8-3-2-1-1\ A.pdf 9-8-3-2-1-1_A.pdf;

mv 9-8-3-2-1-1\ B.pdf 9-8-3-2-1-1_B.pdf;

mv 9-8-3-2-1-1\ C.pdf 9-8-3-2-1-1_C.pdf;

mv 9-9-2-2-1-1\ A.pdf 9-9-2-2-1-1_A.pdf;

mv 9-9-2-2-1-1\ B.pdf 9-9-2-2-1-1_B.pdf;

mv 9-9-2-2-1-1\ C.pdf 9-9-2-2-1-1_C.pdf;

mv 9-9-2-2-1-1\ D.pdf 9-9-2-2-1-1_D.pdf;

mv 9-9-9-3-3-1-1-1.pdf 9-9-9-3-3-1-1-1.pdf;

mv Dessin1Attempt2add.pdf Dessin1Attempt2add.pdf;

mv Dessin1Attempt2.pdf Dessin1Attempt2.pdf;

mv Dessin1attempt.pdf Dessin1attempt.pdf;

mv .DS_Store .DS_Store;

mv Fourth\ Gamma5\ Attempt.pdf Fourth_Gamma5_Attempt.pdf;

mv New\ 16-4-1-1-1-1.pdf New_16-4-1-1-1-1.pdf;

mv New\ 18-9-2-2-2-1-1-1.pdf New_18-9-2-2-2-1-1-1.pdf;

mv New\ 24-8-3-3-3-3-1-1-1-1.pdf New_24-8-3-3-3-3-1-1-1-1.pdf;

mv New\ 27-3-1-1-1-1-1-1.pdf New_27-3-1-1-1-1-1-1.pdf;

mv New\ 3-3-3-3.pdf New_3-3-3-3.pdf;

mv New\ 6-6-6-6-3-3-3-3.pdf New_6-6-6-6-3-3-3-3.pdf;

mv New\ 9-1-1-1.pdf New_9-1-1-1.pdf;

mv New\ 9-9-3-3-3-3-3-3\ Second\ Attempt.pdf New_9-9-3-3-3-3-3-3_Second_Attempt.pdf;

mv Other\ Index\ 60\ Third\ Attempt.pdf Other_Index_60_Third_Attempt.pdf;
